Modeling Word Emotion in Historical Language: Quantity Beats Supposed Stability in Seed Word Selection

To understand historical texts, we must be aware that language -- including the emotional connotation attached to words -- changes over time. In this paper, we aim at estimating the emotion which is associated with a given word in former language stages of English and German. Emotion is represented following the popular Valence-Arousal-Dominance (VAD) annotation scheme. While being more expressive than polarity alone, existing word emotion induction methods are typically not suited for addressing it. To overcome this limitation, we present adaptations of two popular algorithms to VAD. To measure their effectiveness in diachronic settings, we present the first gold standard for historical word emotions, which was created by scholars with proficiency in the respective language stages and covers both English and German. In contrast to claims in previous work, our findings indicate that hand-selecting small sets of seed words with supposedly stable emotional meaning is actually harmful rather than helpful.

==> figs/documents.tex <==
\begin{figure}[t]\hspace*{-5pt}
\begin{tikzpicture}[scale=0.95]
\begin{axis}[
     x tick label style={rotate=90},
           xmin=1690,xmax=2000,xtick={1690,1730,1780,1830,1890,1950,2000},xticklabels={1690s,1730s,1780s,1830s,1890s,1950s,2000s},
    ybar=0pt,bar width=2pt,
    ylabel={tokens in corpus},ylabel near ticks, 
    legend style={at={(0,1)},anchor=north west},
]
\addplot table[col sep = tab, x=decade, y=coha]{figs/words-per-year.csv};
\addplot table[col sep = tab, x=decade, y=dta]{figs/words-per-year.csv};
\legend{COHA,DTA}
\end{axis}
\end{tikzpicture}\hspace*{5pt}
\caption{\label{fig:words-per-decade}Number of tokens per decade in the COHA and DTA corpora as used in our experiments. Each of the red DTA bars represent the sum of three decades.}
%DTA values are shown only for the middle one of three decades (added up).
\end{figure}

==> figs/words_per_decade.tex <==
\label{sec:corpora}
\begin{figure}[t]\hspace*{-5pt}
\begin{tikzpicture}[scale=0.95]
\begin{axis}[
     x tick label style={rotate=90},
           xmin=1690,xmax=2000,xtick={1690,1730,1780,1830,1890,1950,2000},xticklabels={1690s,1730s,1780s,1830s,1890s,1950s,2000s},
    ybar=0pt,bar width=2pt,
    ylabel={tokens in corpus},ylabel near ticks, 
    legend style={at={(0,1)},anchor=north west},
]
\addplot[color=blue] table[col sep = tab, x=decade, y=coha]{figs/words-per-year.csv};
\addplot[fill=red, color=red] table[col sep = tab, x=decade, y=dta]{figs/words-per-year.csv};
\legend{COHA,DTA}
\end{axis}
\end{tikzpicture}\hspace*{5pt}
\caption{\label{fig:words-per-decade}Number of tokens per decade in the COHA and DTA corpora as used in our experiments. DTA bars  each represent three decades (added up).}
%DTA values are shown only for the middle one of three decades (added up).
\end{figure}

==> tabs/deprecated_diachron.tex <==
% \begin{table*}[tbh]
% \centering
% \begin{tabular}{|c|c|c|cc|}\hline
% Language	&	Induction Method 		& Seed Lexicon 	& \svdpmi & SGNS \\ \hline\hline
% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{English}}}
% 			&	\textsc{kNN} 						& full			& \heatc{0.307}	& \textbf{\heatc{0.365}}	\\ 
% 			&	\textsc{ParaSimNum} 			& full				& \heatc{0.348}	& \heatc{0.361}	\\ 
% 			&	\textsc{RandomWalkNum} 	& full				& \heatc{0.351}	& \heatc{0.361}	\\ \cline{2-5}
% 			&	\textsc{kNN} 						& limited 		& \heatd{0.273}	& \heatd{0.153}\\
% 			&	\textsc{ParaSimNum}			& limited 		& \heatd{0.295}	& \heatd{0.232}\\
% 			&	\textsc{RandomWalkNum}	& limited 		&\textbf{ \heatd{0.305}}	& \heatdtraingle{0.039}\\ \hline\hline
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{German}}}
% 			&	\textsc{kNN} 						& full				& \heate{0.366}	& \heate{0.263}\\
% 			&	\textsc{ParaSimNum} 			& full				& \textbf{\heate{0.384}}	& \heate{0.214}\\
% 			&	\textsc{RandomWalkNum} 	& full				& \heate{0.302}	& \heate{0.273}\\  \hline
% \end{tabular}
% \caption{Results of the diachronic evaluation in Pearson's $r$ (averaged over all three VAD dimensions). Values are \textcolor{black!50}{s}\textcolor{black!60}{h}\textcolor{black!70}{a}\textcolor{black!80}{d}\textcolor{black!90}{e}\textcolor{black!100}{d} to emphasize relative performance. The best system for each language and seed selection strategy (\textit{full} vs. \textit{limited}) is in \textbf{bold}, only systems marked with `$^\triangle$' are significantly different from the best system (p $<$ 0.05).\label{tab:diachron}}
% \end{table*}
